Searching Search Spaces: Meta-evolving a Geometric Encoding for Neural Networks

In evolutionary policy search, neural networks are usually represented using a direct mapping: each gene encodes one network weight. Indirect encoding methods, where each gene can encode for multiple weights, shorten the genome to reduce the dimensions of the search space and better exploit permutations and symmetries. The Geometric Encoding for Neural network Evolution (GENE) introduced an indirect encoding where the weight of a connection is computed as the (pseudo-)distance between the two linked neurons, leading to a genome size growing linearly with the number of genes instead of quadratically in direct encoding. However GENE still relies on hand-crafted distance functions with no prior optimization. Here we show that better performing distance functions can be found for GENE using Cartesian Genetic Programming (CGP) in a meta-evolution approach, hence optimizing the encoding to create a search space that is easier to exploit. We show that GENE with a learned function can outperform both direct encoding and the hand-crafted distances, generalizing on unseen problems, and we study how the encoding impacts neural network properties.

==> macros.tex <==
\newcommand{\fulltitle}{Harry Potter and the Use of Structures in\\Evolution Strategies for Neural Policy Search}


\newcommand{\tocite}[1]{ \textcolor{red}{[#1]} }
\newcommand{\addlink}[2]{\href{#1}{#2}\footnote{\url{#1}}}
\def\code#1{\texttt{#1}}

\newcommand{\pt}[1]{\todo[backgroundcolor=blue]{PT}\textcolor{blue}{[\textbf{PT}: #1]}}
\newcommand{\er}[1]{\todo[backgroundcolor=red]{ER}\textcolor{red}{[\textbf{ER}: #1]}}
\newcommand{\dgw}[1]{\todo[backgroundcolor=green]{DGW}\textcolor{green}{[\textbf{DGW}: #1]}}

\newcommand{\addref}[1]{\todo[backgroundcolor=orange]{Ref}\textcolor{orange}{[\textbf{Add ref}: #1]}}


\newcommand{\censor}[1]{#1}



\newcommand{\neat}{NEAT}
\newcommand{\hyperneat}{HyperNEAT}
\newcommand{\es}{evolution strategies}
\newcommand{\snes}{SNES}
\newcommand{\xnes}{XNES}
\newcommand{\enes}{eNES}
\newcommand{\cmaes}{CMA-ES}
\newcommand{\sepcmaes}{Sep-CMA-ES}
\newcommand{\lmmaes}{LM-MA-ES}
\newcommand{\openaies}{OpenAI ES}
\newcommand{\canonical}{Canonical ES}
\newcommand{\direct}{direct encoding}
\newcommand{\ars}{Augmented Random Search}
\newcommand{\mapelites}{MAP-Elites}
\newcommand{\cmame}{CMA-ME}
\newcommand{\pgame}{PGA-ME}



\newcommand{\gene}{GENE}
\newcommand{\longgene}{Geometric Encoding for Neural network Evolution}
\newcommand{\coordsnet}{GENE}
\newcommand{\xdgene}{XD-GENE}
\newcommand{\ltwogene}{L2-GENE}
\newcommand{\grngene}{tag-GENE}
\newcommand{\pltwogene}{pL2-GENE}
\newcommand{\coordinates}{\textit{coordinates}}
\newcommand{\distfunc}{\textit{distance function}}

\newcommand{\dqnes}{DQNES}
\newcommand{\elitES}{ElitES}
\newcommand{\customes}{Custom ES}

\newcommand{\berl}{\code{BERL}}
\newcommand{\cambrian}{\code{Cambrian.jl} }

\newcommand{\openaipaper}{\citep{salimansEvolutionStrategiesScalable2017}}
\newcommand{\canonicalpaper}{\citep{chrabaszczBackBasicsBenchmarking2018} }
\newcommand{\nespaper}{\citep{wierstraNaturalEvolutionStrategies2014}}
\newcommand{\aleguidelines}{\citep{machadoRevisitingArcadeLearning2017}}


\newcommand{\iif}{\Leftrightarrow}

\newcommand{\norm}[1]{\|#1\|}
\newcommand{\carlies}{CARLIES}
\newcommand{\jedi}{JEDi}
\newcommand{\longjedi}{Quality with Just Enough Diversity}
\newcommand{\boldjedi}{Quality with \textbf{J}ust \textbf{E}nough \textbf{Di}versity}

\newcommand{\wtf}{WTFS}
\newcommand{\longwtf}{Weighted Target Fitness Score}

\newcommand{\gdr}{GDR}
\newcommand{\longgdr}{Genetic Drift Regularization}

\newcommand{\sgdr}{GDR²}
\newcommand{\longsgdr}{Squared Genetic Drift Regularization}

\newcommand{\trgdr}{TR-GDR}
\newcommand{\longtrgdr}{Trust Region Genetic Drift Regularization}

\newcommand{\mujoco}{\textsc{MuJoCo}}

\newcommand{\halfcheetah}{\textsc{HalfCheetah}}
\newcommand{\walker}{\textsc{Walker2D}}
\newcommand{\hopper}{\textsc{Hopper}}
\newcommand{\humanoid}{\textsc{Humanoid}}
\newcommand{\swimmer}{\textsc{Swimmer}}
\newcommand{\ant}{\textsc{Ant}}
\newcommand{\antmaze}{\textsc{AntMaze}}
\newcommand{\pointmaze}{\textsc{PointMaze}}


\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\wrt}{\emph{w.r.t.}}
\newcommand{\etc}{\emph{e.t.c.}}
\newcommand{\onemax}{\textsc{OneMax}}
\newcommand{\leadingones}{\textsc{LeadingOnes}}
\newcommand{\procgen}{\textsc{ProcGen}}
\newcommand{\cartpole}{\textsc{CartPole}}
\newcommand{\acrobot}{\textsc{Acrobot}}
\newcommand{\pendulum}{\textsc{Pendulum}}
\newcommand{\qm}[1]{``#1''}
\newcommand{\note}[1]{{\color{blue}#1}}
\newcommand{\honemax}{H2}
\newcommand{\hleadingones}{H5}
\newcommand{\red}[1]{{\color{red}#1}}


==> manuscript_macros.tex <==
\newcommand{\fulltitle}{Harry Potter and the Use of Structures in\\Evolution Strategies for Neural Policy Search}


\newcommand{\tocite}[1]{ \textcolor{red}{[#1]} }
\newcommand{\addlink}[2]{\href{#1}{#2}\footnote{\url{#1}}}
\def\code#1{\texttt{#1}}

\newcommand{\pt}[1]{\todo[backgroundcolor=blue]{PT}\textcolor{blue}{[\textbf{PT}: #1]}}
\newcommand{\er}[1]{\todo[backgroundcolor=red]{ER}\textcolor{red}{[\textbf{ER}: #1]}}
\newcommand{\dgw}[1]{\todo[backgroundcolor=green]{DGW}\textcolor{green}{[\textbf{DGW}: #1]}}

\newcommand{\addref}[1]{\todo[backgroundcolor=orange]{Ref}\textcolor{orange}{[\textbf{Add ref}: #1]}}


\newcommand{\censor}[1]{#1}


\titleformat{\subsubsection}
{\normalfont\normalsize\itshape}{\thesubsubsection}{1em}{}
\renewcommand{\thesubsubsection}{\alph{subsubsection}}

\newcommand{\subsubsubsection}[1]{\paragraph{#1}}


\newcommand{\neat}{NEAT}
\newcommand{\hyperneat}{HyperNEAT}
\newcommand{\es}{evolution strategies}
\newcommand{\snes}{SNES}
\newcommand{\xnes}{XNES}
\newcommand{\enes}{eNES}
\newcommand{\cmaes}{CMA-ES}
\newcommand{\sepcmaes}{Sep-CMA-ES}
\newcommand{\openaies}{OpenAI ES}
\newcommand{\canonical}{Canonical ES}
\newcommand{\direct}{direct encoding}
\newcommand{\ars}{Augmented Random Search}
\newcommand{\mapelites}{MAP-Elites}


\newcommand{\gene}{GENE}
\newcommand{\longgene}{Geometric Encoding for Neural network Evolution}
\newcommand{\coordsnet}{GENE}
\newcommand{\xdgene}{XD-GENE}
\newcommand{\ltwogene}{L2-GENE}
\newcommand{\grngene}{tag-GENE}
\newcommand{\pltwogene}{pL2-GENE}
\newcommand{\coordinates}{\textit{coordinates}}
\newcommand{\distfunc}{\textit{distance function}}

\newcommand{\dqnes}{DQNES}
\newcommand{\elitES}{ElitES}
\newcommand{\customes}{Custom ES}

\newcommand{\berl}{\code{BERL}}
\newcommand{\cambrian}{\code{Cambrian.jl} }

\newcommand{\openaipaper}{\citep{salimansEvolutionStrategiesScalable2017}}
\newcommand{\canonicalpaper}{\citep{chrabaszczBackBasicsBenchmarking2018} }
\newcommand{\nespaper}{\citep{wierstraNaturalEvolutionStrategies2014}}
\newcommand{\aleguidelines}{\citep{machadoRevisitingArcadeLearning2017}}


\newcommand{\iif}{\Leftrightarrow}

\newcommand{\norm}[1]{\|#1\|}
\newcommand{\carlies}{CARLIES}
\newcommand{\jedi}{JEDi}
\newcommand{\longjedi}{Quality with Just Enough Diversity}
\newcommand{\demons}{DEMONS}
\newcommand{\longdemons}{Dispersion Estimation with Monte-Carlo Sampling}


\newcommand{\gdr}{GDR}
\newcommand{\longgdr}{Genetic Drift Regularization}

\newcommand{\sgdr}{GDR²}
\newcommand{\longsgdr}{Squared Genetic Drift Regularization}

\newcommand{\trgdr}{TR-GDR}
\newcommand{\longtrgdr}{Trust Region Genetic Drift Regularization}

\newcommand{\mujoco}{\textsc{MuJoCo}}

\newcommand{\halfcheetah}{\textsc{HalfCheetah}}
\newcommand{\walker}{\textsc{Walker2D}}
\newcommand{\hopper}{\textsc{Hopper}}
\newcommand{\humanoid}{\textsc{Humanoid}}
\newcommand{\swimmer}{\textsc{Swimmer}}
\newcommand{\ant}{\textsc{Ant}}
\newcommand{\pointmaze}{\textsc{PointMaze}}


\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\wrt}{\emph{w.r.t.}}
\newcommand{\etc}{\emph{e.t.c.}}
\newcommand{\onemax}{\textsc{OneMax}}
\newcommand{\leadingones}{\textsc{LeadingOnes}}
\newcommand{\procgen}{\textsc{ProcGen}}
\newcommand{\cartpole}{\textsc{CartPole}}
\newcommand{\acrobot}{\textsc{Acrobot}}
\newcommand{\pendulum}{\textsc{Pendulum}}
\newcommand{\qm}[1]{``#1''}
\newcommand{\note}[1]{{\color{blue}#1}}
\newcommand{\honemax}{H2}
\newcommand{\hleadingones}{H5}
\newcommand{\red}[1]{{\color{red}#1}}

\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\lnof}[1]{\ensuremath{\ln\left(#1\right)}}
\newcommand{\expof}[1]{\ensuremath{\exp\left(#1\right)}}
\newcommand{\powerof}[2]{\ensuremath{\left(#1\right)^{#2}}}
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\expect}{\ensuremath{\mathbb{E}}}
\newcommand{\expectof}[1]{\ensuremath{\expect{}\left(#1\right)}}
\newcommand{\proba}{\ensuremath{\mathbb{P}}}
\newcommand{\probaof}[1]{\ensuremath{\proba{}\left(#1\right)}}
\newcommand{\probaofgiven}[2]{\ensuremath{\proba{}\left(#1\;\middle|\;#2\right)}}
\newcommand{\union}[2]{\ensuremath{\bigcup\limits_{#1}^{#2}}}
\newcommand{\sumc}[2]{\ensuremath{\sum_{#1}^{#2}}} %
\newcommand{\intc}[2]{\ensuremath{\int_{#1}^{#2}}} %
\newcommand{\indic}[1]{\ensuremath{\boldsymbol{1}\left(#1\right)}} %
\newcommand{\intrange}[2]{\ensuremath{\left\{#1,\dots,#2\right\}}}
\newcommand{\eqdef}{\ensuremath{\stackrel{\text{def}}{=}}}
\newcommand{\bigo}{\ensuremath{\mathcal{O}}}
\newcommand{\bigoof}[1]{\ensuremath{\bigo{}\left(#1\right)}}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclareMathOperator\erf{erf}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\newcommand{\csta}{\ensuremath{4}}
\newcommand{\cstatimestwo}{\ensuremath{8}}
\newcommand{\cstaminusone}{\ensuremath{3}}
\newcommand{\cstaminustwo}{\ensuremath{2}}
\newcommand{\cstb}{\ensuremath{2}}
\newcommand{\cst}[1]{\ensuremath{C_{#1}}}
\newcommand{\gammamax}{\ensuremath{0.57}}
\newcommand{\cstlemmathree}{\ensuremath{\tilde{C}}}
\newcommand{\npopmin}{\ensuremath{2}} %
\newcommand{\tmin}{\ensuremath{2}} %
\newcommand{\deltamax}{\ensuremath{0.5}} %

\newcommand{\npop}{\ensuremath{n}} %
\newcommand{\nresampling}{\ensuremath{n_{\text{RS}}}}
\newcommand{\scalingfactor}{\ensuremath{\alpha}}
\newcommand{\nbits}{\ensuremath{N}} %
\newcommand{\budget}{\ensuremath{B}} %
\newcommand{\samplingstrategy}{\ensuremath{\mathcal{S}}}
\newcommand{\pbcomplexity}[2]{\ensuremath{H^{#1,#2}}}%
\newcommand{\meansymbol}[1]{\ensuremath{f}} %
\newcommand{\mean}[1]{\ensuremath{\meansymbol{}_{#1}}}%
\newcommand{\empiricalmean}[3]{\ensuremath{\hat{\meansymbol{}}_{#1}^{#2,#3}}}%
\newcommand{\ttotal}{\ensuremath{N_{\text{non-term}}}}%
\newcommand{\tremain}{\ensuremath{N_{\text{remain}}}}%
\newcommand{\samplessymbol}{\ensuremath{u}}
\newcommand{\nones}[1]{\ensuremath{D^{#1}}}%
\newcommand{\opt}{\ensuremath{\text{opt}}}
\newcommand{\pes}{\ensuremath{\text{pes}}}
\newcommand{\xpesrv}[1]{\ensuremath{X^{\pes{}}_{#1}}}%
\newcommand{\xoptrv}[1]{\ensuremath{X^{\opt{}}_{#1}}}%
\newcommand{\xpes}[1]{\ensuremath{x^{\pes{}}_{#1}}}%
\newcommand{\xopt}[1]{\ensuremath{x^{\opt{}}_{#1}}}%
\newcommand{\observationsymbol}[1]{\ensuremath{O}}
\newcommand{\observationof}[1]{\ensuremath{\observationsymbol{}\left(#1\right)}}%
\newcommand{\nsamples}[3]{\ensuremath{\samplessymbol{}_{#1}^{#2,#3}}}%
\newcommand{\nsamplesstar}[3]{\ensuremath{\samplessymbol{}_{#1}^{*}(#3)}}%
\newcommand{\nsamplesinit}[2]{\ensuremath{U_{#1}^{#2}}}%
\newcommand{\nsamplesinitmax}[1]{\ensuremath{U^{#1}}}%
\newcommand{\boundsymbol}{\ensuremath{\beta}}
\newcommand{\bound}[3]{\ensuremath{\boundsymbol{}\left(#1,#3\right)}}%
\newcommand{\boundbarsymbol}{\ensuremath{\bar{\beta}}}
\newcommand{\boundbar}[3]{\ensuremath{\boundbarsymbol{}\left(#1,#3\right)}}%
\newcommand{\hucb}[2]{\ensuremath{h_{*}^{#1,#2}}} %
\newcommand{\llcb}[2]{\ensuremath{l_{*}^{#1,#2}}} %
\newcommand{\hucbshort}[2]{\ensuremath{h^{#2}}}
\newcommand{\llcbshort}[2]{\ensuremath{l^{#2}}}
\newcommand{\maxc}[2]{\ensuremath{\left[#1\wedge#2\right]}} %

\newcommand{\individuals}[1]{\ensuremath{\textsc{Ind}^{#1}}} %
\newcommand{\topset}[1]{\ensuremath{\textsc{Top}^{#1}}} %
\newcommand{\botset}[1]{\ensuremath{\textsc{Bot}^{#1}}} %
\newcommand{\goodset}[1]{\ensuremath{\textsc{Good}^{#1}}} %
\newcommand{\badset}[1]{\ensuremath{\textsc{Bad}^{#1}}} %
\newcommand{\highset}[2]{\ensuremath{\textsc{High}^{#1,#2}}} %
\newcommand{\lowset}[2]{\ensuremath{\textsc{Low}^{#1,#2}}} %
\newcommand{\aboveset}[2]{\ensuremath{\textsc{Above}^{#1,#2}}} %
\newcommand{\middleset}[2]{\ensuremath{\textsc{Middle}^{#1,#2}}} %
\newcommand{\belowset}[2]{\ensuremath{\textsc{Below}^{#1,#2}}} %

\newcommand{\failgen}[1]{\ensuremath{F^{#1}}}%
\newcommand{\failgenstep}[2]{\ensuremath{F^{#1}_{#2}}}%
\newcommand{\cross}[2]{\ensuremath{\textsc{Cross}^{#1,#2}}}
\newcommand{\crossind}[3]{\ensuremath{\textsc{Cross}_{#1}^{#2,#3}}}
\newcommand{\needy}[3]{\ensuremath{\textsc{Needy}_{#1}^{#2,#3}}}
\newcommand{\terminate}[2]{\ensuremath{\textsc{Term}^{#1,#2}}}

